Multilayer Dataflow: Orchestrate Butterfly Sparsity to Accelerate Attention Computation

Recent neural networks (NNs) with self-attention exhibit competitiveness across different AI domains, but the essential attention mechanism brings massive computation and memory demands. To this end, various sparsity patterns are introduced to reduce the quadratic computation complexity, among which the structured butterfly sparsity has been proven efficient in computation reduction while maintaining model accuracy. However, its complicated data accessing pattern brings utilization degradation and makes parallelism hard to exploit in general block-oriented architecture like GPU. Since the reconfigurable dataflow architecture is known to have better data reusability and architectural flexibility in general NN-based acceleration, we want to apply it to the butterfly sparsity for acquiring better computational efficiency for attention workloads. We first propose a hybrid butterfly-sparsity network to obtain better trade-offs between attention accuracy and performance. Next, we propose a scalable multilayer dataflow method supported by coarse-grained streaming parallelism designs, to orchestrate the butterfly sparsity computation on the dataflow array. The experiments show that compared with Jetson Xavier NX, our design has a speedup of up to $14.34\times$ ($9.29\times$ on average) as well as $11.14\times$ energy efficiency advancement in attention workloads. In comparison with SOTA attention accelerators of the same peak performance, our dataflow architecture acquires $2.38\times$-$4.7\times$ efficiency improvement as well as $6.60\times$-$15.37\times$ energy reduction with butterfly sparsity optimization.

==> related_work.tex <==
\section{Related Work} % wu haibin
\label{sec:related_work}
The sparse attention involves limiting each token to attend to a subset of the other tokens to reduce the computation and memory requirements. One implementation of the sparse attention is called the dynamic sparsity, where the matrix is determined based on the content of the sequence. Ham et al. propose an algorithm called the Efficient Greedy Candidate Search \cite{simict}, which dynamically prunes entries based on their greedy score importance. Kitaev et al. \cite{simict} propose to use Locality Sensitive Hashing (LSH) to infer content-based sparsity patterns for attention. Qu et al. use low-rank linear transformations to estimate attention scores \cite{simict}, then dynamically select the sparse attention pattern by top-k research. However, the aforementioned approach is not scalable and application-dependent. The other implementation called the static sparsity can address these drawbacks by applying a general sparse pattern to different attention matrices. Common static sparse attention patterns are often a combination of several basic sparse patterns in figure 1. For example, Child et al. \cite{simict} firstly introduce a sparsity model which combines sliding and dilated sliding window attention, showing that the sparse attention is sufficient to get state-of-the-art results in modeling long sequences \cite{simict}. Zaheer et al. \cite{simict} come up with a sparse attention model called Big Bird by combining the sliding window attention, global attention and random attention. In Longformer \cite{simict}, Beltagy et al. propose the Global + Sliding Window sparse pattern to scale linearly with the input sequence, making it efficient for longer sequences.


